Algorithms for Lipschitz Learning on Graphs

We develop fast algorithms for solving regression problems on graphs where one is given the value of a function at some vertices, and must find its smoothest possible extension to all vertices. The extension we compute is the absolutely minimal Lipschitz extension, and is the limit for large $p$ of $p$-Laplacian regularization. We present an algorithm that computes a minimal Lipschitz extension in expected linear time, and an algorithm that computes an absolutely minimal Lipschitz extension in expected time $\widetilde{O} (m n)$. The latter algorithm has variants that seem to run much faster in practice. These extensions are particularly amenable to regularization: we can perform $l_{0}$-regularization on the given values in polynomial time and $l_{1}$-regularization on the initial function values and on graph edge weights in time $\widetilde{O} (m^{3/2})$.

==> experiments.tex <==
\section{Experiments with \Rnote{what are we calling lex?}}
\label{sec:webspam}

\Rnote{we need to state that dataset is available online, hosted by us?}
\Rnote{should we describe where we got hold of the data}

\Rnote{we could add some more motivation? e.g. similar to introduction of Zhou}

\Rnote{I haven't covered how we resolve ambiguities. Also I worry a little about the inf interval vs fin interval cases}

We study the issue of detecting spam webpages using the dataset \texttt{webspam-uk2006-2.0} described in \cite{Castillo2006}. This collection includes 11,402 hosts, out of which 7,473 (65.5 \%) are labeled, thisÊeither as \texttt{spam} or \texttt{normal}. Of the hosts 1924 are labeled spam (25.7 \% of all labels). We consider the problem of classifying hosts as spam or not, given only a small fraction of the labels for training.

We construct a directed graph on the set of hosts. In fact, each host corresponds to a collection of web pages. We add a directed edge from host A and to host B, with weight equal to the number of links from the pages of host A to the pages of host B. We take the length of an edge to be the inverse of its weight. To allow easy comparison with the algorithms of \cite{Zhou2007}, we select a strongly connected component of the graph to use for our experiment. We use the largest strongly connected component of the graph, which contains 7945 hosts, of which 5552 are labeled as \texttt{spam} or \texttt{normal}. Spam labels amount to 16 \% of all the labels in this subgraph. To create training and test data, for some value $p$ we select at random $p$ \% of the spam labels and $p$ \% of the normal labels  to use for training. The remaining labels are used for testing. We report results for $p = 5$ and $p = 20$.

Because the label set is highly unbalanced, it is hard to discern our ability to identify spam from overall classification error.  Instead, we use measures of precision and recall. Recall is the fraction of spam-labeled hosts in the test set that we classify as spam. Precision is the fraction of spam-classified hosts from the test set that were in fact labeled spam in the ground truth data. By varying the threshold for classifying a host as spam, we can produce different levels of recall.

The among algorithms studied by \cite{Zhou2007}, the top performer was their algorithm based on sampling according to a random-walk which moves out along in-links from other hosts. We compare their algorithm with the classification we get by using directed lex-minimizing voltages with the convention that \texttt{spam} results in a label of 1 and \texttt{normal} in a label of 0, and that when host A links to host B, the edge gradient is $\frac{v(B) - v(A)}{\len(A,B)}$. This gives the following effects: When unlabeled host A links to spam host B, this is evidence that A is spammy. But when unlabeled host A links to a normal host B, this does not provide evidence that A is normal. When a normal host A links to an unlabeled host B, this is evidence that B is normal, but when a spam host A links to B, this is not evidence that B is spam.

Results are shown in figure \Rnote{todo}. While are not able to reliably classify all hosts, we see that in the range of 10-50 \% recall, we are able to classify spam with precision above 82 \%.

\begin{figure}[ht]
\vspace{-0in}
    \centering
    \includegraphics[scale=0.4]{Experiments/bigwebspam_100runs_5percent.eps}
\includegraphics[scale=0.4]{Experiments/bigwebspam_100runs_20percent.eps}
\vspace{-0in}
\caption{\Rnote{Updated to use 100 runs when available! And elaborate on figure}}
    \label{fig:experiment_image}
\end{figure}

In appendix \Rnote{todo}, we show the performance of our algorithm and that of \cite{Zhou2007} both with link directions reversed, as well as the performance of Laplacian inference, all of which are significantly worse.

==> minvc_tcdag.tex <==
\section{Minimum Vertex Cover in Transitively Closed DAG}
\label{sec:minvc-tcdag}

To prove Theorem~\ref{thm:minvc-tcdag} we use a classic result by K\"{o}nig \cite{Trevisan11}.

\begin{theorem}{\bf K\"{o}nig's Theorem.}
\label{thm:konig}
In a bipartite graph $G$, the size of the minimum vertex cover is equal to the size of the maximum matching. Given a maximum matching, a vertex cover of the graph may be computed in linear time.
\end{theorem}

\begin{definition}{\bf The $\setof{s,t}$-graph of a bipartite graph.}
Let $G = (L \union R, E)$ be a bipartite graph, with $L$ and $R$ disjoint and $E \subseteq L \times R$.

The $\setof{s,t}$-graph $G'=(V',E')$ of $G$ is a directed graph whose vertex set $V'$ is given by $V' = \setof{s,t} \union L \union R$, where $s$ is a new source vertex and $t$ is a new sink vertex. We create an edge set $E'$ which contains for every $l \in L$ an edge $(s,l)$ with capacity 1, for every $r \in R$ an edge $(r,t)$ with capacity 1, for every edge $(l,r) \in E$, and edge $(l,r)$ with capacity $+\infty$.
\end{definition}

The following is a standard result  \cite{Trevisan11}.

\begin{lemma}{\bf Reducing Maximum Bipartite Matching to Maximum $s$-$t$ Flow.}
\label{lem:bipmm-maxflow}
Let $G = (L \union R, E)$ be a bipartite graph, with $L$ and $R$ disjoint and $E \subseteq L \times R$, and let $G'$ be the associated $\setof{s,t}$-graph. Given an integral maximum flow in $G'$, we can compute in linear time a maximum matching in $G$.
\end{lemma}

\begin{definition}{\bf The double graph of a DAG.}
\label{def:doublegraph}
Given a DAG $G = (V,E)$, construct the following bipartite graph $H = (L \union R, \Ehat)$: For every $v \in V$ put a vertex $(v,1)$ in $L$ and a vertex $(v,2)$ in $R$. For every edge $(u,v) \in E$ put edge $((u,1) , (v,2))$ in $\Ehat$. We call $H$ the double graph of $G$.
\end{definition}


\begin{proofof}{of Theorem \ref{thm:minvc-tcdag}}
Given a transitively closed DAG $G = (V,E)$, construct the associated double graph $H$ of $G$, as per Definition~\ref{def:doublegraph}.
We claim that $\minVC(H) \geq \minVC(G)$. Proof: Given a vertex cover $U$ in $H$ construct a vertex cover $U'$ in $G$ by
\[
U' = \setof{ v \in G : (v,1) \in U \text{ or } (v,2) \in U }.
\]
Clearly, $U'$ is a vertex cover in $G$, and $\sizeof{U'} \leq \sizeof{U}$.

We claim that $\minVC(G) \geq \maxMatch(H)$. Proof: Consider any matching $M$ in $H$. Look at the corresponding edges $M'$ in $G$. $M'$ is a subgraph of $G$, where every vertex has both in-degree and out-degree at most 1. Thus $M'$ is a collection of disjoint directed paths. Consider any such path of length $l$. It involves $l+1$ vertices and by transitive closure, these vertices form an $(l+1)$ clique. Thus a vertex cover of $G$ must contain at least $l$ vertices from this clique. Thus every vertex cover in $G$ is at least as large as the matching in $H$.
Now, by Theorem~\ref{thm:konig}, we have $\maxMatch(H) = \minVC(H)$, so we conclude that $\minVC(H) = \minVC(G)$. 
By Lemma~\ref{lem:bipmm-maxflow}, we can compute a maximum matching in $H$ in time $\tilde{O}(m_{H} \min\setof{ n_{H}^{2/3}, m_{H}^{1/2} })$ using the Goldberg-Rao algorithm \cite{Goldberg98} for maximum flow. From this maximum matching, by Theorem~\ref{thm:konig}, we can compute a minimum vertex cover of $H$ in $O(m_{H})$ time.  Finally, as we observed above, we can construct a vertex cover of $G$ from the vertex cover in $H$ in $O(n_{G})$ time.

\end{proofof}

We can also show the following stronger version of Theorem~\ref{thm:minvc-tcdag}.

\begin{theorem}
\label{thm:minvc-tcdag-implicit}
There exists an algorithm that for any DAG $G$ computes a minimum vertex cover of the \emph{transitive closure} of $G$ in time
$\tilde{O}(m_{G} \min\setof{ n_{G}^{2/3}, m_{G}^{1/2} })$.
\end{theorem}

To prove this version, we state a slightly stronger version of K\"{o}nig's theorem \cite{Trevisan11}.

\begin{theorem}{\bf K\"{o}nig's Theorem, version II.}
\label{thm:konigcut}
In a bipartite graph $G$, the size of the minimum vertex cover is equal to the size of the minimum $s$-$t$ cut of the associated $\setof{s,t}$-graph $G'$. Given a minimum $s$-$t$ cut in $G'$, we can find in linear time a vertex cover of $G$.
\end{theorem}

\begin{definition}{\bf The TC-$\setof{s,t}$ graph of a DAG.}
\label{def:tc-st-graph}
Given a DAG $G = (V,E)$, construct the following capacitated graph $H = (L \union R, \Ehat)$
\begin{enumerate}
\item
For every $v \in V$ put a vertex $(v,1)$ in $L$ and a vertex $(v,2)$ in $R$.
\item
For every $v \in V$ put an edge $(s,(v,1))$ in $\Ehat$ with capacity $1$, and an edge $((v,2),t)$ in $\Ehat$ with capacity 1.
\item
For every edge $(u,v) \in E$ put edge $((u,1) , (v,2))$ in $\Ehat$ with capacity $+\infty$.
\item
For every $v \in V$, put an edge $((v,2),(v,1))$ in $\Ehat$ with capacity $+\infty$.
\end{enumerate}
We call $H$ the TC-$\setof{s,t}$ graph of $G$.
\end{definition}

The construction described above would be the $\setof{s,t}$-graph of the double graph of $G$, except for the addition of edges of the form $((v,2),(v,1))$.

\begin{lemma}
\label{lem:tc-st-graph-cuts}
For a DAG $G = (V,E)$, let $G_{TC}$ be its transitive closure. Let $H$ be the TC-$\setof{s,t}$ graph $G$. Let $H_{TC}$ be the $\setof{s,t}$-graph of the double graph of $G_{TC}$. The every minimum $s$-$t$ cut of $H$ is a minimum $s$-$t$ cut of $H_{TC}$. 
\end{lemma}

\begin{proof}
First we will show that each minimum $s$-$t$ cut of $H = (L \union R, E_{H})$ is a cut of the same value in $H_{TC} =  (L \union R, E_{TC})$. 

Consider a minimum $s$-$t$ cut in $H$ given by the source-side set $S_{s} \supseteq \setof{s} $ and the sink-side set $S_{t}  \supseteq \setof{t} $.
Let $L_{i} = L \intersect S_{i}$ for $i \in \setof{s,t}$, and let $R_{i} = R \intersect S_{i}$ for $i \in \setof{s,t}$. The cut with $S_{s} = \setof{s}$ has finite value, so all minimum cuts must have finite value. So in $H$, only edges in $\setof{s} \times L$ and $R \times \setof{t}$ are cut. These edges also appear in $H_{TC}$. Hence the only way that the cut $(S_{s},S_{t})$ could have a different value in $H_{TC}$ is if a transitive closure edge contributes to the cut-value in $H_{TC}$.

Suppose for a contradiction that a transitive closure edge $((v_{0},1),(v_{k},2)) \in E_{TC}$ contributes to the value of the cut  $(S_{s},S_{t})$. As the edge contributes to the value of the cut, $(v_{0},1) \in L_{s}$ and $(v_{k},2) \in R_{t}$. Let $P = (v_{0},v_{1},\ldots,v_{k})$ be a path from $v_{0}$ to $v_{k}$ in G. This path must exist for the transitive closure edge $(v_{0},v_{k})$ to appear in $G_{TC}$ and hence $((v_{0},1),(v_{k},2))$ in $H_{TC}$.

Because the cut $(S_{s},S_{t})$ has finite value in $H$ no edge of $E_{H}$ crosses from $L_{s}$ to $R_{t}$, since this would give the cut value $+\infty$, and similarly no edge crosses from $R_{s}$ to $L_{t}$. Using these two facts, we will show that $(v_{k},2) \in R_{s}$.

Edge $(v_{0},v_{1})$ appears in $G$, so $((v_{0},1),(v_{1},2))$ appears in $H$, and $(v_{0},1) \in L_{s}$ so $(v_{1},2)$ appears in $R_{s}$. As edge $((v_{1},2),(v_{1},1))$ is in $H$, it must be that $(v_{1},1) \in L_{s}$. Repeating this argument along the path of vertices to $(v_{k},2)$, we get that $(v_{k},2) \in R_{s}$, which contradicts $(v_{k},2) \in R_{t}$, so our assumption that the transitive closure edge contributed to the cut must be wrong. Thus we have shown that any minimum cut of $H$ is a cut of the same value in $H_{TC}$. This also implies $\minVC(H_{TC}) \leq \minVC(H)$.

Now, we will show that no cut in $H_{TC}$ achieves a lower value. By the strong maximum flow-minimum cut duality, $\minVC(H_{TC})  = \maxFlow(H_{TC})$. Consider any integral flow $\ff$ in $H$. We claim that you can re-route this flow in $H_{TC}$ without increasing the congestion. Look at a path decomposition of the flow $\ff$. Consider a flow on a single path $(s,(v_{0},1), (v_{1},2),(v_{1},1),\ldots,(v_{k},2),t)$. To route this in $H_{TC}$, simply send the flow along the path $(s,(v_{0},1),(v_{k},2),t)$, which must appear in $H_{TC}$ by the transitive closure property. This will not increase congestion, as we congest edges $(s,(v_{0},1))$ and $((v_{k},2),t)$ by the same amount we did before, and edge $((v_{0},1),(v_{k},2))$ has capacity $\infty$. But this means that
\[
\minVC(H) = \maxFlow(H) \leq \maxFlow(H_{TC}) = \minVC(H_{TC}).
\]
Now we can conclude that every minimum $s$-$t$ cut in $H$ is also a minimum $s$-$t$ cut in $H_{TC}$.
\end{proof}


\begin{proofof}{of Theorem \ref{thm:minvc-tcdag-implicit}}
The proof is essentially the same as that of Theorem~\ref{thm:minvc-tcdag}, but we observe that by Lemma~\ref{lem:tc-st-graph-cuts} and Theorem~\ref{thm:konigcut}, it suffices to compute a minimum cut of the TC-$\setof{s,t}$ graph $H$ of a DAG $G$ to find a vertex cover of the transitive closure of $G$. From the TC-$\setof{s,t}$ graph construction, it is clear that $H$ contains $n_{H}=O(n_{G})$ vertices and $m_{H}=O(m_{G})$ edges, so we can compute a minimum cut in $H$ in $\tilde{O}(m_{G} \min\setof{ n_{G}^{2/3}, m_{G}^{1/2} })$ time using the Goldberg-Rao maximum flow algorithm.
\end{proofof}

